Federated Learning Meets Fairness and Differential Privacy

Deep learning's unprecedented success raises several ethical concerns ranging from biased predictions to data privacy. Researchers tackle these issues by introducing fairness metrics, or federated learning, or differential privacy. A first, this work presents an ethical federated learning model, incorporating all three measures simultaneously. Experiments on the Adult, Bank and Dutch datasets highlight the resulting ``empirical interplay" between accuracy, fairness, and privacy.

==> FPFL-framework.tex <==
    
    \begin{figure}[!t]
        \centering
        \fbox{
        {
    
    \begin{minipage}{0.45\textwidth}
    \begin{center}
        \textbf{FPFL Framework}
    \end{center}
    
    \begin{enumerate}[noitemsep, leftmargin=*]
        \item \textbf{Initialization}
        \item \textbf{Local Training Process.} Each agent $i\in\mathbb{A}$, invokes Algorithm~\ref{algo::P1}
        
        \item \textbf{Local Training Process.} Each agent $i\in\mathbb{A}$, invokes Algorithm~\ref{algo::P2}
        \item Local training process ends
        \item \textbf{Model Aggregation.} Aggregator computes and then broadcasts an overall model
        \item Agents re-initialize their local models with the overall model received
        \item Repeat steps from 3 to 6 until a sufficient overall accuracy is reached
    \end{enumerate}

     \end{minipage}}
        }
        \caption{FPFL Framework}
         \label{fig::FPFL-framework}
    \end{figure}
